ACE-Router: Generalizing History-Aware Routing from MCP Tools to the Agent Web

With the rise of the Agent Web and Model Context Protocol (MCP), the agent ecosystem is evolving into an open collaborative network, exponentially increasing accessible tools. However, current architectures face severe scalability and generality bottlenecks. To address this, we propose ACE-Router, a pipeline for training history-aware routers to empower precise navigation in large-scale ecosystems. By leveraging a dependency-rich candidate Graph to synthesize multi-turn trajectories, we effectively train routers with dynamic context understanding to create the plug-and-play Light Routing Agent. Experiments on the real-world benchmarks MCP-Universe and MCP-Mark demonstrate superior performance. Notably, ACE-Router exhibits critical properties for the future Agent Web: it not only generalizes to multi-agent collaboration with minimal adaptation but also maintains exceptional robustness against noise and scales effectively to massive candidate spaces. These findings provide a strong empirical foundation for universal orchestration in open-ended ecosystems.

==> table/scale.tex <==
\begin{table}[h]
    \centering
    % 如果表格太宽，取消下面这一行的注释来自动缩放
    % \resizebox{\columnwidth}{!}{
    \begin{tabular}{lccc}
        \toprule
        \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c}{\textbf{Avg. Accuracy (\%)}} \\
        \cmidrule(lr){2-4}
        & \textbf{1.5B} & \textbf{4B} & \textbf{8B} \\
        \midrule
        MCP-Universe &  &  &  \\
        MCP-Mark &  & &  \\
        \bottomrule
    \end{tabular}
    % }
    \caption{Performance scaling of the router across Qwen3 different model sizes (1.5B, 4B, and 8B). We report the Average Accuracy on the evaluation set.}
    \label{tab:router_scaling}
\end{table}
